Sub-Picosecond Carrier Dynamics Explored using Automated High-Throughput Studies of Doping Inhomogeneity within a Bayesian Framework

Bottom-up production of semiconductor nanomaterials is often accompanied by inhomogeneity resulting in a spread in electronic properties which may be influenced by the nanoparticle geometry, crystal quality, stoichiometry or doping. Using photoluminescence spectroscopy of a population of more than 20,000 individual Zn-doped GaAs nanowires, we reveal inhomogeneity in, and correlation between doping and nanowire diameter by use of a Bayesian statistical approach. Recombination of hot-carriers is shown to be responsible for the photoluminescence lineshape; by exploiting lifetime variation across the population, we reveal hot-carrier dynamics at the sub-picosecond timescale showing interband electronic dynamics. High-throughput spectroscopy together with a Bayesian approach are shown to provide unique insight in an inhomogeneous nanomaterial population, and can reveal electronic dynamics otherwise requiring complex pump-probe experiments in highly non-equilibrium conditions.

==> header.tex <==
\usepackage[utf8]{inputenc}
\usepackage{amsmath} % Math symbols
\usepackage{amssymb}
\usepackage{color}            % For highlighting text
\usepackage{soul}           % For \hl command
\usepackage{graphicx}
\usepackage{subfig}
\usepackage[version=4]{mhchem}
\SectionNumbersOn

% Added in revision
\sethlcolor{yellow}
\newcommand{\REVISION}{}
%

\setkeys{acs}{email = false}
\newcommand{\onlinecite}[1]{\hspace{-1 ex} \nocite{#1}\citenum{#1}} 
% set figure width
\newcommand{\width}{0.95\columnwidth}

% Results
\newcommand{\BESOsep}{$0.326_{0.312}^{0.341}$\,eV}
\newcommand{\SRV}{$1.17_{0.41}^{2.60}\times10^{6}$\,cm/s}
\newcommand{\pdoping}{$9.67_{5.08}^{17.76}\times10^{19}$\,cm$^{-3}$}
\newcommand{\diameter}{$76_{68}^{84}$\,nm}
\newcommand{\usedwires}{11,487}
\newcommand{\mcmc}{1,100,000}
\newcommand{\mcmcFilter}{203,512}
\newcommand{\T}{$1984_{1741}^{2240}$\,K}
\newcommand{\ta}{$193_{112}^{347}$\,fs}
\newcommand{\pdeg}{$1.5\times10^{20}$\,cm$^{-3}$}
\newcommand{\slope}{$0.91_{0.90}^{0.92}$}
\newcommand{\meff}{0.118}
\newcommand{\tamx}{1\,ps}
\newcommand{\tauFit}{1.10$\pm$0.02\,ps}
\newcommand{\pturnp}{$2.3\times10^{20}$\,cm$^{-3}$}
\newcommand{\IQEmx}{$2\%$}
\newcommand{\alphaSampling}{$2\times10^{-15}$}

%%%%%%%%%%%%%% META
\title{Sub-Picosecond Carrier Dynamics Explored using Automated High-Throughput Studies of Doping Inhomogeneity within a Bayesian Framework}

\author{Ruqaiya Al-Abri}
\email{ruqaiya.al-abri@postgrad.manchester.ac.uk}
\author{Nawal Al Amairi}
\author{Stephen Church}
\affiliation{Department of Physics and Astronomy and the Photon Science Institute, University of Manchester, Oxford Road, Manchester, M13 9PL, United Kingdom}
\author{Conor Byrne}
\affiliation{Department of Chemistry, University of Manchester, Oxford Road, Manchester, M13 9PL, United Kingdom}
\author{Sudhakar Sivakumar}
\affiliation{Department of Physics and NanoLund, Lund University, Box 118, SE-221 00, Sweden}
\author{Alex Walton}
\affiliation{Department of Chemistry, University of Manchester, Oxford Road, Manchester, M13 9PL, United Kingdom}
\author{Martin H. Magnusson}
\affiliation{Department of Physics and NanoLund, Lund University, Box 118, SE-221 00, Sweden}
\author{Patrick Parkinson}
\affiliation{Department of Physics and Astronomy and the Photon Science Institute, University of Manchester, Oxford Road, Manchester, M13 9PL, United Kingdom}

